The role of mechano-electric feedbacks and hemodynamic coupling in scar-related ventricular tachycardia

Mechano-electric feedbacks (MEFs), which model how mechanical stimuli are transduced into electrical signals, have received sparse investigation by considering electromechanical simulations in simplified scenarios. In this paper, we study the effects of different MEFs modeling choices for myocardial deformation and nonselective stretch-activated channels (SACs) in the monodomain equation. We perform numerical simulations during ventricular tachycardia (VT) by employing a biophysically detailed and anatomically accurate 3D electromechanical model for the left ventricle (LV) coupled with a 0D closed-loop model of the cardiocirculatory system. We model the electromechanical substrate responsible for scar-related VT with a distribution of infarct and peri-infarct zones. Our mathematical framework takes into account the hemodynamic effects of VT due to myocardial impairment and allows for the classification of their hemodynamic nature, which can be either stable or unstable. By combining electrophysiological, mechanical and hemodynamic models, we observe that all MEFs may alter the propagation of the action potential and the morphology of the VT. In particular, we notice that the presence of myocardial deformation in the monodomain equation may change the VT basis cycle length and the conduction velocity but do not affect the hemodynamic nature of the VT. Finally, nonselective SACs may affect wavefront stability, by possibly turning a hemodynamically stable VT into a hemodynamically unstable one and vice versa.

==> EMmodel_lv.tex <==
% This block of code is essential to use the [resume] flag for subequations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\user@resume{resume}
\def\user@intermezzo{intermezzo}
%
\newcounter{previousequation}
\newcounter{lastsubequation}
\newcounter{savedparentequation}
\setcounter{savedparentequation}{1}
%
\renewenvironment{subequations}[1][]{%
      \def\user@decides{#1}%
      \setcounter{previousequation}{\value{equation}}%
      \ifx\user@decides\user@resume
           \setcounter{equation}{\value{savedparentequation}}%
      \else
      \ifx\user@decides\user@intermezzo
           \refstepcounter{equation}%
      \else
           \setcounter{lastsubequation}{0}%
           \refstepcounter{equation}%
      \fi\fi
      \protected@edef\theHparentequation{%
          \@ifundefined {theHequation}\theequation \theHequation}%
      \protected@edef\theparentequation{\theequation}%
      \setcounter{parentequation}{\value{equation}}%
      \ifx\user@decides\user@resume
           \setcounter{equation}{\value{lastsubequation}}%
         \else
           \setcounter{equation}{0}%
      \fi
      \def\theequation  {\theparentequation  \alph{equation}}%
      \def\theHequation {\theHparentequation \alph{equation}}%
      \ignorespaces
}{%
%  \arabic{equation};\arabic{savedparentequation};\arabic{lastsubequation}
  \ifx\user@decides\user@resume
       \setcounter{lastsubequation}{\value{equation}}%
       \setcounter{equation}{\value{previousequation}}%
  \else
  \ifx\user@decides\user@intermezzo
       \setcounter{equation}{\value{parentequation}}%
  \else
       \setcounter{lastsubequation}{\value{equation}}%
       \setcounter{savedparentequation}{\value{parentequation}}%
       \setcounter{equation}{\value{parentequation}}%
  \fi\fi
%  \arabic{equation};\arabic{savedparentequation};\arabic{lastsubequation}
  \ignorespacesafterend
}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newlength{\temp}
\newcommand{\EPfirstline}{
	J \EPchim \left[ \EPCm \dfrac{\partial u}{\partial t} + \EPIion(u, \boldsymbol{w}) + \EPISAC(u, \mecF) \right] - \nabla \cdot ( J \mecF^{-1} \EPdiffTens \, \mecF^{-T} \nabla u) = J \EPchim \EPIapp(t)
}
\settowidth{\temp}{$\EPfirstline$}
\newcommand{\widthbox}[1]{\makebox[\temp][l]{$#1$}}

\begin{subequations}\label{eqn: EM}
\begin{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\Monodomain_{\text{gMEF-full, SAC}})
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
\begin{cases}\label{eqn: EP}
\EPfirstline & \text{in } \Omega_0 \times (0,T], \\
\widthbox{\dfrac{\partial \boldsymbol{w}}{\partial t} - \EPrhsGating(u, \boldsymbol{w}) = \boldsymbol{0}} & \text{in } \Omega_0 \times (0,T], \\ %\\[0.2cm]
\left( J \mecF^{-1} \EPdiffTens \, \mecF^{-T} \nabla u \right) \cdot \mecNref = 0  & $on$ \; \partial \Omega_0 \times (0, T],
\end{cases}
\end{align}
\end{subequations}
%in $\Omega_0 \times (0, T)$, with $u = u_0$ and $\boldsymbol{w} = \boldsymbol{w}_0$ in $\Omega_0$ at time $t=0$.
\begin{subequations}[resume]
\begin{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\PhyAct)\label{eqn: Act}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\quad
\widthbox{ \frac{\partial \ActStateHF}{\partial t} = \ActRhs\left(\ActStateHF,\Cai,\SL, \frac{\partial \SL}{\partial t}\right) } & \text{in } \Omega_0 \times (0,T],
%- \epsSL^2 \Delta \SL + \SL   = \SL_0 \sqrt{\IIVf}
%& \text{in } \Omega_0 \times (0,T), \\
%\displaystyle
%\epsSL^2 \nabla \SL \cdot \mathbf{N} = 0
%& \text{on } \partial\Omega_0 \times (0,T), \\
\end{align}
\end{subequations}
%in $\Omega_0 \times (0, T)$, with $\ActStateHF(0) = \ActStateHF_0$ in $\Omega_0$ at time $t=0$.
\begin{subequations}[resume]
\begin{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\PhyMec)\label{eqn: Mec}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
\begin{cases}
\widthbox{\rho_{\text{s}} \dfrac{\partial^2 \displ}{\partial t^2} - \nabla \cdot \tenspiola(\displ, \Tens(\ActStateHF,\SL)) = \boldsymbol{0} } & \text{in } \Omega_0 \times (0,T], \\
\tenspiola(\displ, \Tens(\ActStateHF,\SL)) \mecNref =
\BCmecKepiTens \displ +
\BCmecCepiTens \dfrac{\partial \displ}{\partial t} & $on$ \; \GammaEpi \times (0, T], \\
\tenspiola(\displ, \Tens(\ActStateHF,\SL)) \mecNref = -\PLV(t) \, J \mecF^{-T} \mecNref & $on$ \; \GammaEndo \times (0, T], \\
%\tenspiola(\displ, \Tens(\ActStateHF,\SL)) \mecNref = \displaystyle \frac{| J \mecF^{-T} \mecNref |}{\int_{\GammaBase} | J \mecF^{-T} \mecNref | d \Gamma_0}\int_{\GammaEndo} \PLV(t) J \mecF^{-T} \mecNref d \Gamma_0 \\
\tenspiola(\displ, \Tens(\ActStateHF,\SL)) \mecNref = \displaystyle | J \mecF^{-T} \mecNref | \BCmecVbaseLV(t)
& $on$ \; \GammaBase \times (0, T], \\[0.2cm]
\end{cases}
\end{align}
\end{subequations}
%\todo[inline]{FR: qui seconodo me non è chiara la dipendenza da $\XiHat$ (sembra quasi una variabile spaziale). Puttosto toglierei le parentesi (spiegare qui il ruolo di xi non è facile).}
%in $\Omega_0 \times (0, T)$, with $\displ = \displ_0$ and $\dfrac{\partial \displ}{\partial t} = \Dot{\displ}_0$ in $\Omega_0$ at time $t=0$.
\begin{subequations}[resume]
\begin{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\PhyCirc)\label{eqn: Circ}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\quad
\widthbox{\dfrac{d \Circ(t)}{d t} = \CircRhs(t, \Circ(t), \PLV(t)) } & \text{for } t \in (0,T],
\end{align}
\end{subequations}
%for $t \in (0, T)$, with $\CircOne(0)=\CircOneInit$.
\begin{subequations}[resume]
\begin{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\PhyCoupl)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\quad
\widthbox{\VLV(\Circ(t)) = \VLVthreedim(\displ(t)) } & \text{for } t \in (0,T],
\end{align}
\end{subequations}
%for $t \in (0, T)$


==> pictures/header_slides.tex <==
\RequirePackage[T1]{fontenc}
\PassOptionsToPackage{sfdefault, lining}{FiraSans}
\RequirePackage{FiraSans}

\usepackage{sfmath} % to force sans serif in math mode
\renewcommand{\familydefault}{\sfdefault} % per usare il sans serif nel testo

\usepackage{amssymb}
\usepackage{bbm} %per la funzione indicatrice
\usepackage{mathrsfs} %per mathscr

\usepackage{xcolor}
%\usepackage{siunitx} 
%\usepackage{tabularx}

\input{../macros.tex}
